BridgeRouter: Gain-Aware Instance Routing over Cross-Modal Bridge Portfolios

Lightweight representation bridges make pretrained, task-adapted EEG foundation models executable on other biosignal modalities without retraining their backbones. However, selecting a single bridge pathway globally assigns every instance to the same transfer route and ignores complementary errors across routes. We therefore formulate multi-bridge transfer as an instance-level algorithm-selection problem and introduce BridgeRouter, a gain-aware router over a portfolio of frozen cross-modal pathways. A validation-selected Single Best Solver (SBS) serves as a protected default route. During training, task labels are used to compute the reduction in negative log-likelihood provided by each alternative route relative to the SBS, and a lightweight MLP predicts these route-specific gains from a target-modality representation extracted by a frozen encoder. At inference, BridgeRouter observes only the target modality, requires neither EEG, task labels, nor predictions from all candidate routes, and executes exactly one bridge pathway: the route with the largest predicted gain when that gain exceeds a validation-calibrated threshold, and the SBS otherwise. We evaluate seven EEG foundation-model bridge pathways for EMG-based freezing-of-gait detection on FOG and ECG-based sleep classification on ISRUC. Across five seeds, BridgeRouter achieves $81.38\pm1.11\%$ balanced accuracy on FOG, improving over the BIOT SBS by $11.49$ percentage points, and $62.92\pm2.17\%$ on ISRUC, improving over the CBraMod SBS by $3.83$ points. Per-instance bridge oracles reach $99.96\%$ and $78.61\%$, respectively, revealing substantial remaining portfolio headroom. These results show that anchor-relative gain prediction can convert complementary cross-modal bridge behavior into deployable instance-level routing improvements while retaining single-route inference.

==> old_version.tex <==
We compare our task-label-free Transfer-Aware Bridge Router with three groups of baselines. First, we evaluate every individual BioX-style bridge as a fixed inference pathway. We additionally report the single best solver (SBS), selected exclusively by validation balanced accuracy and then frozen for test evaluation. The SBS is the primary task-label-free comparison because it uses the same frozen encoder, bridge portfolio, and downstream classifiers as our method, but applies one globally selected bridge to every instance.

Second, we evaluate two label-free routing controls. The \emph{competence-only} router selects the route with the highest predicted teacher confidence, whereas the \emph{transfer-only} router selects routes using only predicted teacher-to-bridge discrepancy and prediction-flip probability. These controls isolate the two components of our transfer-aware score.

Third, we report task-label-supervised references, including a target-only linear classifier, a target-only MLP, the Gain-only Router, and strict adaptation of EEG-AS~\cite{zhang2026eegas}. These methods use downstream task labels or label-derived correctness and gain targets during training and are therefore reported as supervised contextual references rather than directly comparable task-label-free baselines. Finally, we report per-instance bridge oracles to quantify portfolio complementarity. These oracles are non-deployable and are not used for model selection.

\paragraph{Implementation Details.}
We use NormWear and HuBERT-ECG as the target-modality encoders for EMG and ECG, respectively, and seven pretrained EEG foundation models as candidate receivers. For each receiver, we freeze both pretrained encoders and train a lightweight bridge on temporally paired EEG--target-modality windows. Bridge checkpoints are selected on the validation split and subsequently frozen for all routing experiments.

The selected FOG bridge positions are reported in Table~\ref{tab:bridge_layers_emg}. Validation-set auditing identifies severe prediction collapse in the LaBraM, EEGPT, and REVE bridge routes. We therefore retain BIOT, CBraMod, CSBrain, and BENDR as the compact four-route portfolio for the task-label-free router. The collapsed routes remain included when reporting the complete seven-bridge results and oracle, but they are excluded from the compact routing portfolio according to this validation-defined rule.

\begin{table}[t]
\caption{Selected source and destination layers for the NormWear-to-EEG-FM bridges on FOG.}
\label{tab:bridge_layers_emg}
\begin{center}
\small
\begin{tabular}{lll}
\multicolumn{1}{c}{\bf ROUTE} &
\multicolumn{1}{c}{\bf SOURCE} &
\multicolumn{1}{c}{\bf DESTINATION}
\\ \hline
NormWear $\to$ LaBraM  & block 4 & layer 1 \\
NormWear $\to$ EEGPT   & block 5 & layer 5 \\
NormWear $\to$ REVE    & block 7 & layer 21 \\
NormWear $\to$ BIOT    & block 6 & layer 2 \\
NormWear $\to$ CBraMod & block 4 & layer 6 \\
NormWear $\to$ CSBrain & block 9 & layer 6 \\
NormWear $\to$ BENDR   & block 9 & layer 6 \\
\end{tabular}
\end{center}
\end{table}

\begin{table}[t]
\caption{Selected source and destination layers for the HuBERT-ECG-to-EEG-FM bridges on ISRUC.}
\label{tab:bridge_layers_ecg}
\begin{center}
\small
\begin{tabular}{lll}
\multicolumn{1}{c}{\bf ROUTE} &
\multicolumn{1}{c}{\bf SOURCE} &
\multicolumn{1}{c}{\bf DESTINATION}
\\ \hline
HuBERT-ECG $\to$ LaBraM  & block 0 & layer 3 \\
HuBERT-ECG $\to$ EEGPT   & block 1 & layer 6 \\
HuBERT-ECG $\to$ REVE    & block 6 & layer 21 \\
HuBERT-ECG $\to$ BIOT    & block 1 & layer 3 \\
HuBERT-ECG $\to$ CBraMod & block 2 & layer 4 \\
HuBERT-ECG $\to$ CSBrain & block 7 & layer 11 \\
HuBERT-ECG $\to$ BENDR   & block 6 & layer 7 \\
\end{tabular}
\end{center}
\end{table}

For FOG, the task-label-free router takes the 768-dimensional pooled representation from NormWear block~6 as input. A shared MLP with hidden dimensions 256 and 128, GELU activations, and dropout of 0.2 predicts three route-specific transfer signals: teacher confidence, normalized Jensen-Shannon divergence, and prediction-flip probability. For route $k$, these estimates are combined as
\[
\hat{s}_{ik}
=
\hat{c}_{ik}(1-\hat{f}_{ik})
-
\hat{d}_{ik},
\]
and the route with the largest score is selected.

The router is trained on $D_{\mathrm{pair}}$ using signals derived only from paired EEG--EMG predictions. Neither task labels nor label-derived correctness, rescue, harm, or gain targets are accessible during router training or inference. Checkpoint selection is based on held-out transfer-signal prediction loss rather than downstream classification performance. At inference time, the router observes only the target-modality input and executes the selected frozen bridge and receiver. We evaluate five router seeds, 42-46, while keeping the bridge portfolio fixed.

\paragraph{Evaluation Metrics.}
We report accuracy, balanced accuracy, macro F1, and weighted F1 for downstream classification. Balanced accuracy is the primary metric because of class imbalance. For routing analyses, we additionally report the number of anchor errors rescued, anchor successes harmed, and the resulting net change in correctly classified instances. For a selected route $k$, a rescue occurs when the anchor is incorrect and route $k$ is correct; a harm occurs when the anchor is correct and route $k$ is incorrect. All mean and standard-deviation results are computed over five router seeds.

\subsection{FOG Results}

\subsubsection{Direct EEG Foundation-Model Performance}

Table~\ref{tab:fog_direct_eeg} reports the performance obtained when each frozen EEG foundation model directly processes EEG from $D_{\mathrm{new}}$. BIOT is the strongest individual EEG model, reaching 76.89\% balanced accuracy. However, the seven-model oracle reaches 97.98\%, indicating substantial instance-level diversity even before cross-modal transfer.

\begin{table}[t]
\caption{Direct-EEG performance on the FOG12 test set.}
\label{tab:fog_direct_eeg}
\begin{center}
\small
\begin{tabular}{lrrrr}
\multicolumn{1}{c}{\bf MODEL} &
\multicolumn{1}{c}{\bf ACC.} &
\multicolumn{1}{c}{\bf BACC.} &
\multicolumn{1}{c}{\bf F1-M} &
\multicolumn{1}{c}{\bf F1-W}
\\ \hline
LaBraM  & 67.58 & 66.02 & 66.19 & 67.24 \\
EEGPT   & 73.09 & 72.89 & 72.66 & 73.18 \\
REVE    & 73.27 & 72.59 & 72.61 & 73.26 \\
BIOT    & \textbf{76.96} & \textbf{76.89} & \textbf{76.61} & \textbf{77.04} \\
CBraMod & 63.08 & 60.54 & 60.43 & 62.00 \\
CSBrain & 61.55 & 58.25 & 57.62 & 59.59 \\
BENDR   & 59.03 & 58.50 & 58.39 & 59.18 \\ \hline
Oracle  & 98.17 & 97.98 & -- & -- \\
\end{tabular}
\end{center}
\end{table}

\subsubsection{Individual Cross-Modal Bridges}

Table~\ref{tab:fog_bridges} evaluates the seven fixed NormWear-to-EEG-FM routes. BIOT is selected as the SBS because it obtains the highest validation balanced accuracy. On the test set, it reaches 69.89\% balanced accuracy. BENDR and CSBrain are the next strongest routes, with 65.96\% and 64.05\%, respectively.

Bridge quality is not determined solely by the direct-EEG performance of the receiver. In particular, BENDR and CSBrain improve over their corresponding direct-EEG models by 7.46 and 5.80 percentage points, whereas EEGPT and REVE experience transfer losses exceeding 21 percentage points. The seven-bridge oracle reaches 99.96\% balanced accuracy, although this near-perfect value is partly driven by complementary class-biased routes and should not be interpreted as achievable routing performance.

\begin{table}[t]
\caption{Performance of the fixed cross-modal bridges on the FOG12 test set. BIOT is the validation-selected SBS.}
\label{tab:fog_bridges}
\begin{center}
\small
\begin{tabular}{lrrrr}
\multicolumn{1}{c}{\bf ROUTE} &
\multicolumn{1}{c}{\bf ACC.} &
\multicolumn{1}{c}{\bf BACC.} &
\multicolumn{1}{c}{\bf F1-M} &
\multicolumn{1}{c}{\bf F1-W}
\\ \hline
LaBraM  & 57.63 & 49.98 & 36.59 & 42.17 \\
EEGPT   & 58.39 & 51.09 & 39.83 & 44.95 \\
REVE    & 42.91 & 50.41 & 31.14 & 26.79 \\
BIOT    & \textbf{69.07} & \textbf{69.89} & \textbf{68.98} & \textbf{69.23} \\
CBraMod & 57.30 & 58.02 & 57.23 & 57.50 \\
CSBrain & 65.07 & 64.05 & 64.10 & 65.00 \\
BENDR   & 65.72 & 65.96 & 65.47 & 65.92 \\ \hline
Oracle  & 99.96 & 99.96 & -- & -- \\
\end{tabular}
\end{center}
\end{table}

\subsubsection{Task-Label-Free Transfer-Aware Routing}

Table~\ref{tab:fog_label_free_router} presents the principal FOG12 result. The BIOT SBS obtains 69.89\% balanced accuracy. Predicting teacher competence alone provides a modest improvement to $70.22\pm0.10\%$. Transfer-only routing substantially changes individual predictions and increases ordinary accuracy, but its mean balanced accuracy remains close to the SBS. This shows that transfer discrepancy alone does not reliably identify the most task-useful route.

Combining predicted competence and transfer risk yields the strongest task-label-free result. Our Transfer-Aware Bridge Router reaches
$71.91\pm0.43\%$ balanced accuracy and
$72.37\pm0.32\%$ accuracy, improving over the BIOT SBS by
$2.02\pm0.43$ percentage points in balanced accuracy. The improvement is observed for all five router seeds.
\begin{table}[t]
\caption{
Task-label-free routing results on the FOG12 test set.
Mean and sample standard deviation are reported over five router seeds.
Rescue and harm are measured relative to the BIOT SBS.
The compact-four oracle is non-deployable.
}
\label{tab:fog_label_free_router}
\begin{center}
\small
\setlength{\tabcolsep}{5pt}

\textbf{(a) Classification performance}
\vspace{2pt}

\begin{tabular}{lrrr}
\multicolumn{1}{c}{\bf METHOD} &
\multicolumn{1}{c}{\bf ACC.} &
\multicolumn{1}{c}{\bf BACC.} &
\multicolumn{1}{c}{\bf $\Delta$ BACC.}
\\ \hline
BIOT SBS
& 69.07
& 69.89
& -- \\

Competence only
& $69.55\pm0.13$
& $70.22\pm0.10$
& $+0.33$ \\

Transfer only
& $71.60\pm0.36$
& $69.90\pm0.48$
& $+0.01$ \\

\textbf{Transfer-Aware}
& $\mathbf{72.37\pm0.32}$
& $\mathbf{71.91\pm0.43}$
& $\mathbf{+2.02\pm0.43}$ \\

Compact-4 oracle
& 93.78
& 93.69
& $+23.80$ \\
\end{tabular}

\vspace{7pt}

\textbf{(b) Routing behavior relative to BIOT}
\vspace{2pt}

\begin{tabular}{lrrr}
\multicolumn{1}{c}{\bf METHOD} &
\multicolumn{1}{c}{\bf RESCUE} &
\multicolumn{1}{c}{\bf HARM} &
\multicolumn{1}{c}{\bf NET CORRECT}
\\ \hline
Competence only
& $120.6\pm27.1$
& $80.6\pm34.3$
& $+40.0\pm10.9$ \\

Transfer only
& $1035.8\pm38.9$
& $826.6\pm47.6$
& $+209.2\pm29.8$ \\

\textbf{Transfer-Aware}
& $\mathbf{580.4\pm69.9}$
& $\mathbf{307.4\pm80.1}$
& $\mathbf{+273.0\pm26.5}$ \\
\end{tabular}

\end{center}
\end{table}

The rescue--harm decomposition explains the source of this improvement. Across the five seeds, Transfer-Aware routing rescues $580.4\pm69.9$ BIOT errors while harming $307.4\pm80.1$ BIOT successes, producing a positive net gain of $273.0\pm26.5$ correctly classified instances. In contrast, transfer-only routing rescues more BIOT errors but also incurs substantially more harms. Teacher competence is therefore necessary to regularize route selection: discrepancy identifies where transfer behavior differs, whereas competence helps determine whether the corresponding receiver is reliable.

Table~\ref{tab:fog_label_free_seeds} shows that the result is stable across random seeds. Test balanced accuracy ranges from 71.17\% to 72.31\%, and every seed improves over the fixed BIOT route.

\begin{table}[t]
\caption{Per-seed stability of the task-label-free Transfer-Aware Bridge Router on FOG12.}
\label{tab:fog_label_free_seeds}
\begin{center}
\small
\begin{tabular}{rrrrr}
\multicolumn{1}{c}{\bf SEED} &
\multicolumn{1}{c}{\bf ACC.} &
\multicolumn{1}{c}{\bf BACC.} &
\multicolumn{1}{c}{\bf $\Delta$ BACC.} &
\multicolumn{1}{c}{\bf NET}
\\ \hline
42 & 72.30 & 72.06 & +2.17 & +267 \\
43 & 71.84 & 71.17 & +1.28 & +229 \\
44 & 72.57 & 71.95 & +2.06 & +289 \\
45 & 72.59 & 72.31 & +2.42 & +291 \\
46 & 72.57 & 72.05 & +2.16 & +289 \\ \hline
Mean $\pm$ SD
& $72.37\pm0.32$
& $71.91\pm0.43$
& $+2.02\pm0.43$
& $+273.0\pm26.5$ \\
\end{tabular}
\end{center}
\end{table}

\subsubsection{Comparison with Task-Label-Supervised References}

Table~\ref{tab:fog_supervised_references} contextualizes the task-label-free result using methods that have access to downstream FOG labels or label-derived route correctness during training. These results are not directly comparable to the proposed label-free setting.

The target-only MLP is the strongest supervised reference, reaching $83.40\pm0.34\%$ balanced accuracy. Strict EEG-AS reaches $82.19\pm0.47\%$, whereas the Gain-only Router reaches $81.38\pm1.11\%$. These results demonstrate that labeled target-modality data provide strong direct supervision. They also define the performance gap between the label-free deployment setting studied here and a conventional supervised target-modality classifier.

\begin{table}[t]
\caption{Task-label-supervised contextual references on FOG12. These methods are not directly comparable to the proposed task-label-free router.}
\label{tab:fog_supervised_references}
\begin{center}
\small
\begin{tabular}{lrr}
\multicolumn{1}{c}{\bf METHOD} &
\multicolumn{1}{c}{\bf TEST BACC.} &
\multicolumn{1}{c}{\bf SUPERVISION}
\\ \hline
Target-only linear
& $79.74\pm0.17$
& Task labels \\
Gain-only Router
& $81.38\pm1.11$
& Label-derived gain \\
Strict EEG-AS
& $82.19\pm0.47$
& Route correctness \\
Target-only MLP
& $\mathbf{83.40\pm0.34}$
& Task labels \\
\end{tabular}
\end{center}
\end{table}

\subsection{Transfer-Loss Analysis on FOG}

\subsubsection{Output-Level Transfer Loss}

We next examine how faithfully each bridge preserves the output behavior of its direct-EEG teacher. For each paired instance, we compare the class distributions produced by direct EEG inference and bridge-based EMG inference. Table~\ref{tab:fog_output_transfer} reports direct-EEG balanced accuracy, bridge balanced accuracy, and the ability of Jensen--Shannon divergence to identify transfer failures among instances that the direct-EEG teacher classifies correctly.

For LaBraM, EEGPT, and REVE, output discrepancy is highly predictive of transfer failure, with AUC values between 0.945 and 0.990. However, the relationship is weaker for CSBrain and BENDR. These two routes obtain higher balanced accuracy after bridge transfer than under direct EEG input, even though the bridge representation is not an exact reconstruction of the EEG representation. Consequently, transfer discrepancy should not be interpreted as task failure in isolation. This finding motivates combining transfer risk with teacher competence in the proposed routing score.

\begin{table}[t]
\caption{Output-level transfer analysis on the FOG12 test set. ``Failure AUC'' measures how well teacher-to-bridge JS divergence identifies bridge failure conditional on a correct direct-EEG prediction.}
\label{tab:fog_output_transfer}
\begin{center}
\small
\begin{tabular}{lrrr}
\multicolumn{1}{c}{\bf ROUTE} &
\multicolumn{1}{c}{\bf EEG BACC.} &
\multicolumn{1}{c}{\bf BRIDGE BACC.} &
\multicolumn{1}{c}{\bf FAILURE AUC}
\\ \hline
LaBraM  & 66.02 & 49.98 & 0.945 \\
EEGPT   & 72.89 & 51.09 & 0.967 \\
REVE    & 72.59 & 50.41 & 0.990 \\
BIOT    & 76.89 & 69.89 & 0.826 \\
CBraMod & 60.54 & 58.02 & 0.831 \\
CSBrain & 58.25 & 64.05 & 0.636 \\
BENDR   & 58.50 & 65.96 & 0.675 \\
\end{tabular}
\end{center}
\end{table}

\subsubsection{Representation-Level Transfer Loss}

To examine whether errors arise immediately at bridge injection or are amplified by the remaining receiver layers, we perform a representation-distance diagnostic for the BIOT pathway. We compare the bridge-generated and direct-EEG representations both at the BIOT destination layer and after propagation through the remaining receiver layers.

As shown in Table~\ref{tab:biot_rep_distance}, the relative $\ell_2$ distance on the test set decreases from 0.6945 at the destination layer to 0.5027 at the final representation, while cosine distance decreases from 0.2262 to 0.1341. Thus, the downstream BIOT layers contract rather than amplify the observed representation discrepancy on average. Nevertheless, a nonzero output JS divergence remains, showing that reduced representation distance does not guarantee identical predictions.

\begin{table}[t]
\caption{BIOT representation-distance diagnostic. ``Dest.'' denotes the bridge injection point, and ``Final'' denotes the representation after the remaining BIOT layers.}
\label{tab:biot_rep_distance}
\begin{center}
\small
\begin{tabular}{lrrrr}
\multicolumn{1}{c}{\bf SPLIT} &
\multicolumn{1}{c}{\bf DEST. NMSE} &
\multicolumn{1}{c}{\bf DEST. COS.} &
\multicolumn{1}{c}{\bf FINAL NMSE} &
\multicolumn{1}{c}{\bf FINAL COS.}
\\ \hline
Pair & 0.4915 & 0.2249 & 0.2428 & 0.1177 \\
Validation & 0.4947 & 0.2263 & 0.2768 & 0.1341 \\
Test & 0.4969 & 0.2262 & 0.2766 & 0.1341 \\
\end{tabular}
\end{center}
\end{table}

\subsection{Portfolio Complementarity and Routing Headroom}

The compact-four oracle reaches 93.69\% balanced accuracy, compared with 69.89\% for the BIOT SBS. Therefore, removing collapsed routes does not eliminate bridge complementarity. The compact portfolio still leaves 23.80 percentage points of oracle headroom over the fixed anchor.

We additionally measure bridge complementarity relative to the stronger supervised target-only MLP. Although the target-only MLP reaches 83.40\% balanced accuracy, combining it with an oracle over the four non-collapsed routes increases balanced accuracy to 97.07\%. Across seeds, approximately 82.77\% of target-only MLP errors are correctly classified by at least one retained bridge. Thus, bridge routes contain complementary decisions even relative to a strong direct target-modality classifier. The practical challenge is not the absence of complementary information, but identifying beneficial switches without task-label supervision.

\subsection{Ablation Study}

\paragraph{Contribution of Transfer Signals.}
The competence-only and transfer-only controls in Table~\ref{tab:fog_label_free_router} isolate the two components of the proposed score. Competence-only routing improves over BIOT by only 0.33 percentage points, suggesting that predicted teacher confidence alone frequently recovers the globally strongest route. Transfer-only routing yields nearly unchanged balanced accuracy because its large number of rescues is offset by a similarly large number of harms. Combining the two signals produces a consistent 2.02-point gain. This supports the design
\[
\text{route utility}
\approx
\text{teacher competence}
-
\text{transfer risk},
\]
rather than either component alone.

\paragraph{Effect of Removing Collapsed Routes.}
Validation predictions identify LaBraM, EEGPT, and REVE as collapsed or nearly collapsed bridge routes: LaBraM and EEGPT overwhelmingly predict Class~0, whereas REVE overwhelmingly predicts Class~1. Although these routes inflate the seven-bridge oracle through complementary class bias, they do not provide reliable general-purpose pathways. We therefore apply the validation-defined filtering rule before training the task-label-free router. The resulting compact-four oracle still reaches 93.69\% balanced accuracy, confirming that substantial complementarity remains among BIOT, CBraMod, CSBrain, and BENDR.

\paragraph{Role of Task-Label Supervision.}
The supervised references outperform the task-label-free router, with the target-only MLP reaching 83.40\% balanced accuracy. This difference does not invalidate the bridge-routing setting: it quantifies the value of target-modality task labels, which are explicitly unavailable to the proposed router. Under the task-label-free constraint, Transfer-Aware routing improves consistently over the fixed BIOT SBS without accessing task labels, route correctness, rescue events, or downstream validation balanced accuracy during router training and checkpoint selection.

\subsection{ISRUC Sleep Classification}
\label{sec:isruc_results}

\paragraph{Individual Bridge Performance.}
Table~\ref{tab:isruc_bridge_performance} reports the final performance of the seven frozen ECG-to-EEG bridge pathways on the 18,920-epoch ISRUC test set. Individual pathway performance varies substantially across foundation models. EEGPT achieves the highest balanced accuracy (BAcc) at 65.1709\%, whereas BENDR, the prespecified Single Best Solver (SBS), achieves the highest accuracy (81.5063\%) and macro-F1 (66.7550\%). These differences indicate that no individual bridge pathway dominates across all evaluation metrics.

\begin{table}[t]
\caption{Performance of the seven frozen ISRUC bridge pathways.}
\label{tab:isruc_bridge_performance}
\begin{center}
\begin{tabular}{lcccc}
\multicolumn{1}{c}{\bf Target FM} &
\multicolumn{1}{c}{\bf Bridge} &
\multicolumn{1}{c}{\bf Acc (\%)} &
\multicolumn{1}{c}{\bf BAcc (\%)} &
\multicolumn{1}{c}{\bf Macro-F1 (\%)} \\
\hline \\
LaBraM  & H0$\rightarrow$L3  & 78.087 & 60.486 & 61.772 \\
CBraMod & H2$\rightarrow$L4  & 78.087 & 59.090 & 60.229 \\
REVE    & H6$\rightarrow$L21 & 79.693 & 61.732 & 63.445 \\
EEGPT   & H1$\rightarrow$L6  & 75.920 & {\bf 65.171} & 65.000 \\
CSBrain & H7$\rightarrow$L11 & 79.096 & 62.905 & 64.438 \\
BENDR   & H6$\rightarrow$L7  & {\bf 81.506} & 64.445 & {\bf 66.755} \\
BIOT    & H1$\rightarrow$L3  & 80.518 & 64.051 & 66.005 \\
\end{tabular}
\end{center}
\end{table}

\paragraph{Portfolio Complementarity.}
Majority voting does not improve over the BENDR SBS in BAcc, whereas
the non-deployable K7 oracle reaches 78.6122\%, revealing substantial
instance-level complementarity across the seven bridge pathways.
This gap motivates instance-wise routing rather than simple aggregation.

\begin{table}[t]
\caption{ISRUC TEST comparison.}
\label{tab:isruc_main_results}
\begin{center}
\begin{tabular}{lccc}
\multicolumn{1}{c}{\bf Method} &
\multicolumn{1}{c}{\bf Acc (\%)} &
\multicolumn{1}{c}{\bf BAcc (\%)} &
\multicolumn{1}{c}{\bf Macro-F1 (\%)} \\
\hline \\
BENDR SBS
& {\bf 81.506}
& 64.445
& {\bf 66.755} \\
EEGPT
& 75.920
& {\bf 65.171}
& 65.000 \\
Majority vote
& 80.973
& 63.770
& 65.903 \\
Adaptive router
& $79.332 \pm 0.420$
& $65.129 \pm 0.347$
& $66.466 \pm 0.454$ \\
Oracle
& 90.127
& 78.612
& 82.976 \\
\end{tabular}
\end{center}
\end{table}


\paragraph{Adaptive Routing.}
The adaptive router achieves $65.1287 \pm 0.3469$\% BAcc across five
seeds, improving over the BENDR SBS by 0.6837 percentage points and
performing comparably to the strongest individual pathway, EEGPT
(65.1709\%), although this improvement does not extend to accuracy or
macro-F1. The substantially higher oracle BAcc of 78.6122\% indicates
that considerable pathway complementarity remains unexploited by the
current router.



\subsection{Ablation Studies}
\label{sec:isruc_ablations}

(these ablations are conducted under ISRUC)

\paragraph{Source Representation.}
Routing performance is relatively stable across the middle HuBERT-ECG
layers, with H3--H5 forming a broad plateau. Although H5 is nominally
best, the difference from the prespecified H4 representation is small.
We therefore retain H4 rather than making a post-hoc layer choice based
on validation performance. Concatenating all layers provides no
additional benefit despite substantially increasing the input
dimension.

\paragraph{Portfolio Size.}
Increasing the portfolio size consistently expands oracle coverage, but
does not monotonically improve the learned router
(Table~\ref{tab:isruc_portfolio}). This distinction suggests that adding
complementary pathways creates additional routing opportunities without
necessarily making those opportunities easier to identify. We retain
the full K7 portfolio to preserve the canonical set of bridge pathways
rather than selecting the validation-optimal subset.

\begin{table}[t]
\caption{ISRUC portfolio-size ablation on VAL. Portfolios are nested
using a TRAIN-only greedy oracle criterion. Router results are mean
$\pm$ sample SD over five seeds.}
\label{tab:isruc_portfolio}
\begin{center}
\begin{tabular}{clcc}
\multicolumn{1}{c}{\bf K} &
\multicolumn{1}{c}{\bf Expert added} &
\multicolumn{1}{c}{\bf Oracle BAcc} &
\multicolumn{1}{c}{\bf Router BAcc} \\
& & \multicolumn{1}{c}{\bf (\%)} &
\multicolumn{1}{c}{\bf (\%)} \\
\hline \\
1 & BENDR   & 64.938 & 64.938 $\pm$ 0.000 \\
2 & EEGPT   & 71.098 & 64.954 $\pm$ 0.037 \\
3 & LaBraM  & 72.717 & 64.938 $\pm$ 0.000 \\
4 & CBraMod & 75.941 & {\bf 65.765 $\pm$ 0.258} \\
5 & CSBrain & 76.475 & 65.613 $\pm$ 0.145 \\
6 & REVE    & 77.719 & 65.610 $\pm$ 0.318 \\
7 & BIOT    & {\bf 78.166} & 65.552 $\pm$ 0.282 \\
\end{tabular}
\end{center}
\end{table}

\paragraph{Routing Design.}
Table~\ref{tab:isruc_routing_ablation} shows that both the routing
target and the decision rule matter. Correctness-based supervision
collapses to the default pathway, while NLL-gain supervision provides
a richer signal for learning when an alternative pathway is useful.
The nonlinear router also outperforms its linear counterpart. Finally,
forcing a switch on every instance removes the benefit of routing,
supporting the use of SBS protection when the predicted gain is
insufficient.

\begin{table}[t]
\caption{Controlled ISRUC H4/K7 routing ablations on VAL.}
\label{tab:isruc_routing_ablation}
\begin{center}
\begin{tabular}{lccc}
\multicolumn{1}{c}{\bf Target / architecture} &
\multicolumn{1}{c}{\bf Acc (\%)} &
\multicolumn{1}{c}{\bf BAcc (\%)} &
\multicolumn{1}{c}{\bf Macro-F1 (\%)} \\
\hline \\
Correctness / MLP
& 81.560 $\pm$ 0.000
& 64.938 $\pm$ 0.000
& 67.439 $\pm$ 0.000 \\
$p_{\mathrm{true}}$ / MLP
& 81.288 $\pm$ 0.178
& 65.044 $\pm$ 0.108
& {\bf 67.441 $\pm$ 0.119} \\
NLL / Linear
& 78.742 $\pm$ 1.515
& 65.142 $\pm$ 0.091
& 66.537 $\pm$ 0.546 \\
NLL / MLP
& 78.602 $\pm$ 0.359
& {\bf 65.552 $\pm$ 0.282}
& 66.823 $\pm$ 0.269 \\
\hline
NLL / MLP, forced
& 77.457 $\pm$ 0.681
& 64.913 $\pm$ 0.224
& 65.844 $\pm$ 0.224 \\
\end{tabular}
\end{center}
\end{table}

\paragraph{Label-Free Transfer Routing.}
We further ask whether pathway selection can be learned without
task-label-derived routing supervision. As a separate development
experiment, we construct transfer signals from each native EEG teacher
and its corresponding bridge: teacher confidence, teacher--bridge
prediction divergence, and prediction disagreement. A router predicts
these quantities from the target-modality representation and uses them
to score the seven bridge pathways. We consider competence-only,
transfer-only, and a prespecified transfer-aware combination of these
signals.

\begin{table}[t]
\caption{Label-free routing on ISRUC VAL. }
\label{tab:isruc_label_free}
\begin{center}
\begin{tabular}{lccc}
\multicolumn{1}{c}{\bf Method} &
\multicolumn{1}{c}{\bf Acc (\%)} &
\multicolumn{1}{c}{\bf BAcc (\%)} &
\multicolumn{1}{c}{\bf Macro-F1 (\%)} \\
\hline \\
BENDR SBS
& 81.560
& 64.938
& 67.439 \\
Supervised NLL
& 78.602 $\pm$ 0.359
& {\bf 65.552 $\pm$ 0.282}
& 66.823 $\pm$ 0.269 \\
\hline
Competence only
& 78.602 $\pm$ 0.089
& 61.580 $\pm$ 0.053
& 63.131 $\pm$ 0.073 \\
Transfer only
& 81.179 $\pm$ 0.159
& 64.544 $\pm$ 0.075
& 66.911 $\pm$ 0.084 \\
Transfer aware
& 78.627 $\pm$ 0.204
& 61.314 $\pm$ 0.247
& 62.844 $\pm$ 0.286 \\
\end{tabular}
\end{center}
\end{table}

The label-free variants do not improve over the SBS
(Table~\ref{tab:isruc_label_free}). In particular, the prespecified
transfer-aware formulation performs substantially below the supervised
NLL-gain router. Transfer-only routing is considerably stronger, but
still falls short of the fixed BENDR pathway. Thus, teacher--bridge
transfer signals alone do not provide a sufficiently reliable basis
for selecting among the heterogeneous bridge pathways.


\subsection{Bridge Heterogeneity and Complementarity}
\label{sec:bridge_heterogeneity}

Table~\ref{tab:bridge_performance} reports all frozen bridge pathways before routing. Performance varies substantially across receivers on both tasks. On FOG, BIOT is the fixed-bridge SBS at 69.89\% BAcc, followed by BENDR and CSBrain, whereas several other routes are near chance or strongly class-biased. Native EEG performance does not fully determine cross-modal performance: EEGPT and REVE lose more than 21 BAcc points after transfer, while BENDR and CSBrain improve by 7.46 and 5.80 points relative to their direct-EEG results. On ISRUC, EEGPT has the highest individual TEST BAcc (65.1709\%), whereas the prespecified BENDR SBS has the highest accuracy (81.5063\%) and macro-F1 (66.7550\%). Thus, no receiver dominates every metric or transfer setting.

These results also distinguish receiver quality from pathway quality. A strong native EEG classifier can be difficult to reach through a learned bridge, while a weaker native receiver can remain competitive after transfer. Consequently, selecting the receiver solely from native EEG performance would discard information about the bridge itself. The relevant portfolio is the set of complete target-encoder--bridge--receiver pathways and their instance-level errors, rather than a ranking of EEG backbones in isolation.

\begin{table}[t]
\caption{Frozen cross-modal bridge performance. Panel (a) reports FOG12 TEST; panel (b) reports authoritative ISRUC TEST.}
\label{tab:bridge_performance}
\centering
\small
\setlength{\tabcolsep}{4.6pt}
\textbf{(a) FOG12}\par\vspace{2pt}
\begin{tabular}{lrrrr}
\hline
Receiver & Accuracy & BAcc & Macro-F1 & Weighted-F1 \\
\hline
LaBraM  & 57.63 & 49.98 & 36.59 & 42.17 \\
EEGPT   & 58.39 & 51.09 & 39.83 & 44.95 \\
REVE    & 42.91 & 50.41 & 31.14 & 26.79 \\
BIOT    & \textbf{69.07} & \textbf{69.89} & \textbf{68.98} & \textbf{69.23} \\
CBraMod & 57.30 & 58.02 & 57.23 & 57.50 \\
CSBrain & 65.07 & 64.05 & 64.10 & 65.00 \\
BENDR   & 65.72 & 65.96 & 65.47 & 65.92 \\
\hline
\end{tabular}

\vspace{6pt}
\textbf{(b) ISRUC}\par\vspace{2pt}
\begin{tabular}{lrrr}
\hline
Receiver & Accuracy & BAcc & Macro-F1 \\
\hline
LaBraM  & 78.0867 & 60.4863 & 61.7722 \\
CBraMod & 78.0867 & 59.0898 & 60.2289 \\
REVE    & 79.6934 & 61.7323 & 63.4451 \\
EEGPT   & 75.9197 & \textbf{65.1709} & 64.9999 \\
CSBrain & 79.0962 & 62.9053 & 64.4379 \\
BENDR   & \textbf{81.5063} & 64.4450 & \textbf{66.7550} \\
BIOT    & 80.5180 & 64.0508 & 66.0054 \\
\hline
\end{tabular}
\end{table}

The pathway errors are also complementary (Table~\ref{tab:portfolio_headroom}). On FOG, we use the realistic compact-four oracle rather than the inflated full-seven oracle, whose near-perfect value is partly produced by complementary class-biased routes. The compact portfolio leaves 23.80 percentage points between the BIOT SBS and its oracle. ISRUC leaves 14.1672 points between BENDR and the K7 oracle; deterministic majority voting reaches only 63.7703\% BAcc, below BENDR. Both tasks therefore contain substantial instance-level bridge complementarity that is not recovered by a fixed SBS or simple aggregation, motivating instance-level routing.

The oracle comparison does not imply that its decisions are available at deployment. It isolates a necessary precondition for routing: alternatives sometimes solve instances missed by the globally preferred pathway. The large gaps on both tasks establish this opportunity, while the majority-vote result shows that diversity alone is insufficient. A deployable router must identify useful alternatives from the target modality without consulting the unknown label.

\begin{table}[t]
\caption{Routing headroom on each final evaluation split. Oracles are non-deployable.}
\label{tab:portfolio_headroom}
\centering
\small
\begin{tabular}{llrrrr}
\hline
Dataset & Portfolio & SBS & SBS BAcc & Oracle BAcc & Headroom \\
\hline
FOG12 TEST & Compact four & BIOT  & 69.89 & 93.69 & $+23.80$ \\
ISRUC TEST & Canonical K7 & BENDR & 64.4450 & 78.6122 & $+14.1672$ \\
\hline
\end{tabular}
\end{table}

% APPENDIX CANDIDATE: full FOG direct-EEG performance table and direct-EEG oracle.
% APPENDIX CANDIDATE: collapsed-route prediction distributions and full-seven FOG oracle.

\subsection{Label-Free Transfer-Aware Routing}
\label{sec:label_free_routing}

We next ask whether pathway utility can be inferred without task-label-derived routing supervision. Table~\ref{tab:label_free_routing} compares the fixed SBS with competence-only, transfer-only, and the prespecified transfer-aware combination. On FOG TEST, competence-only routing gives a small improvement, while transfer-only routing changes many decisions but leaves BAcc effectively unchanged. Combining competence and predicted transfer risk reaches $71.91\pm0.43$\% BAcc, improving on BIOT by $2.02\pm0.43$ points across five seeds.

The FOG router is selected without using downstream classification performance as its training target: predicted native-teacher competence is combined with predicted teacher-to-bridge divergence and prediction-flip probability. The comparison therefore tests whether paired-modality transfer behavior supplies enough information to choose among frozen pathways. The improvement is not driven by one favorable initialization; every one of the five reported seeds exceeds the BIOT SBS in BAcc.

The same general label-free idea does not transfer uniformly to ISRUC's heterogeneous K7 portfolio. On VAL, competence-only and transfer-aware routing fall to $61.5800\pm0.0531$\% and $61.3136\pm0.2472$\% BAcc, respectively, compared with 64.9376\% for BENDR. Transfer-only is closer at $64.5440\pm0.0748$\%, but also remains below the SBS and is retained as a prespecified ablation rather than promoted after observing VAL. The ISRUC result is therefore a substantive negative result: label-free transfer-aware routing improves over the SBS on FOG but does not generalize uniformly across heterogeneous bridge systems.

This contrast is evaluated without opening ISRUC TEST for the label-free lineage. The three label-free scores were fixed before official VAL classification metrics were examined, and VAL outcomes were not used to redefine the score or select transfer-only as a replacement. The comparison is therefore evidence about the portability of the supervision signals, not a post-hoc contest among scoring formulas.

\begin{table}[t]
\caption{Label-free routing over five seeds. FOG uses the compact-four portfolio and is evaluated on TEST; ISRUC uses symmetric K7 routing and is evaluated on VAL.}
\label{tab:label_free_routing}
\centering
\small
\setlength{\tabcolsep}{4.2pt}
\begin{tabular}{lllrrrr}
\hline
Dataset & Method & Split & Accuracy & BAcc & Macro-F1 & $\Delta$BAcc \\
\hline
FOG & BIOT SBS & TEST & 69.07 & 69.89 & 68.98 & -- \\
FOG & Competence only & TEST & $69.55\pm0.13$ & $70.22\pm0.10$ & -- & $+0.33$ \\
FOG & Transfer only & TEST & $71.60\pm0.36$ & $69.90\pm0.48$ & -- & $+0.01$ \\
FOG & Transfer aware & TEST & $\mathbf{72.37\pm0.32}$ & $\mathbf{71.91\pm0.43}$ & -- & $\mathbf{+2.02\pm0.43}$ \\
\hline
ISRUC &
ISRUC & 
ISRUC & 
ISRUC &
\hline
\end{tabular}
\end{table}

FOG rescue--harm behavior clarifies why combining the signals matters. Transfer-only routing rescues $1035.8\pm38.9$ BIOT errors but harms $826.6\pm47.6$ BIOT successes; transfer-aware routing reduces these harmful switches to $307.4\pm80.1$ while retaining $580.4\pm69.9$ rescues, producing a larger net gain of $273.0\pm26.5$ correct predictions.

% APPENDIX CANDIDATE: FOG five-seed transfer-aware routing table.
% APPENDIX CANDIDATE: full FOG rescue/harm table.
% APPENDIX CANDIDATE: ISRUC label-free route frequencies, per-class routes, and per-seed diagnostics.

\subsection{Why Does Label-Free Routing Differ Across Tasks?}
\label{sec:label_free_diagnostics}

On FOG, teacher-to-bridge Jensen--Shannon divergence is strongly associated with transfer failure for some pathways: conditional failure-prediction AUC is 0.945--0.990 for LaBraM, EEGPT, and REVE. The relationship is substantially weaker for CSBrain and BENDR (0.636 and 0.675), whose bridges also outperform their native EEG receivers in BAcc. Transfer discrepancy therefore contains useful pathway-specific information, but is not equivalent to downstream pathway utility. This route dependence is consistent with transfer-only routing's large numbers of both rescues and harms.

In other words, a large teacher--bridge discrepancy can identify an unreliable transfer for routes whose native teacher is already task-competent, but the same discrepancy need not mean that the resulting Bridge prediction is inferior to the available alternatives. The signal is informative conditionally and route by route; treating it as a common absolute utility scale loses this distinction.

ISRUC exposes a different limitation. On the fixed subject-grouped TRAIN diagnostic subset, mean entropy-based competence is perfectly rank-correlated with native-teacher BAcc across FMs (Spearman $\rho=1.00$), but not similarly aligned with Bridge BAcc ($\rho=0.214$). BENDR is the clearest example: its native teacher has extremely low mean entropy competence ($0.022\pm0.026$), despite its Bridge remaining competitive (68.79\% BAcc on this subset). This mismatch is consistent with suppression of useful pathways such as BENDR under the transfer-aware score and suggests that absolute native-teacher competence is not necessarily cross-FM comparable as a measure of Bridge reliability. It does not establish a causal explanation for every routing error.

Together, these diagnostics provide a discussion-ready distinction: transfer-derived signals can be informative within a pathway, while their absolute scales need not be comparable across heterogeneous FM systems.

% APPENDIX CANDIDATE: full FOG output-level transfer-loss table.
% APPENDIX CANDIDATE: BIOT representation-distance diagnostic.
% APPENDIX CANDIDATE: full ISRUC competence-by-FM table, AUCs, utility, and target-score route frequencies.

\subsection{Task-Supervised Gain Routing on ISRUC}
\label{sec:supervised_routing}

Given the limitations of label-free pathway scoring on ISRUC, we next ask how much portfolio headroom can be recovered when task-derived routing supervision is available. The frozen router predicts BENDR-relative NLL gain from the 512-D HuBERT-ECG H4 representation and retains BENDR unless the best predicted alternative exceeds the frozen VAL-selected protection threshold. Five independently trained checkpoints are evaluated once on TEST; no seed selection, ensembling, refitting, or TEST calibration is performed.

Table~\ref{tab:supervised_routing} shows a modest improvement on the primary metric. The adaptive router reaches $65.1287\pm0.3469$\% BAcc, 0.6837 points above the prespecified BENDR SBS. It does not exceed EEGPT's 65.1709\% individual BAcc, and it lowers accuracy and macro-F1 relative to BENDR. Moreover, the K7 oracle remains at 78.6122\% BAcc. Task-derived supervision therefore recovers a modest portion of the available ISRUC routing headroom, but pathway selection remains substantially below the oracle and involves metric tradeoffs.

Relative to the 14.1672-point TEST gap between BENDR and the oracle, the mean BAcc gain recovers 4.83\% of the available headroom. The result is thus neither a general dominance claim nor evidence that complementarity has been exhausted. It shows that label-derived relative gain provides usable routing information on ISRUC, while the remaining gap leaves selective identification of beneficial switches as the central unresolved problem.

\begin{table}[t]
\caption{Authoritative ISRUC TEST comparison. The adaptive router is mean $\pm$ sample SD over seeds 42--46; the oracle is non-deployable.}
\label{tab:supervised_routing}
\centering
\small
\begin{tabular}{lrrr}
\hline
Method & Accuracy & BAcc & Macro-F1 \\
\hline
BENDR SBS & \textbf{81.5063} & 64.4450 & \textbf{66.7550} \\
EEGPT fixed bridge & 75.9197 & 65.1709 & 64.9999 \\
Supervised adaptive router & $79.3319\pm0.4196$ & $65.1287\pm0.3469$ & $66.4662\pm0.4541$ \\
K7 oracle & 90.1268 & 78.6122 & 82.9764 \\
\hline
\end{tabular}
\end{table}

\paragraph{Design checks.}
Development ablations support the frozen ISRUC choices without changing the primary evidence chain. H3--H5 form a broad representation plateau, so we retain prespecified H4 rather than post-hoc H5. Oracle coverage increases with portfolio size, but learned routing is non-monotonic; the VAL-optimal K4 is therefore not promoted over canonical K7. NLL gain is more useful than correctness gain, the nonlinear MLP performs better than the linear NLL predictor, and SBS-protected routing outperforms forced switching. These results justify the selected design but are not independent headline claims.

The complete curves and controlled cells are deferred because their role is methodological rather than to introduce additional primary findings. In particular, nominally better H5 and K4 development values do not replace the prespecified H4/K7 configuration, and the protection comparison is interpreted as evidence for retaining a safe default rather than as a threshold search on TEST.




\subsection{Per-Seed Main Results}
\label{app:per-seed}

Table~\ref{tab:per-seed-main} reports every seed used in the main result.
FOG routing is comparatively stable in both performance and switching rate.
ISRUC is more variable: seed 46 switches on 48.63\% of test instances, whereas
the remaining seeds switch on 1.93--6.24\%.  Importantly, all five corrected
ISRUC runs remain above the validation-selected CBraMod SBS in balanced
accuracy, although seed 45 reduces ordinary accuracy by 113 predictions.

\begin{table*}[t]
\centering
\caption{Per-seed BridgeRouter test diagnostics.  Net correct is measured
relative to the dataset-specific validation-selected SBS.}
\label{tab:per-seed-main}
\small
\begin{tabular}{crrr|rrr}
\hline
& \multicolumn{3}{c}{FOG} & \multicolumn{3}{c}{ISRUC} \\
\hline
Seed & BAcc & Switch & Net correct & BAcc & Switch & Net correct \\
\hline
42 & 81.76 & 68.73\% & $+1045$ & 62.45 & 3.91\% & $+86$ \\
43 & 80.58 & 66.58\% & $+957$  & 63.41 & 5.51\% & $+154$ \\
44 & 79.89 & 67.40\% & $+896$  & 63.41 & 6.24\% & $+139$ \\
45 & 82.52 & 73.93\% & $+1127$ & 59.67 & 1.93\% & $-113$ \\
46 & 82.16 & 72.99\% & $+1110$ & 65.67 & 48.63\% & $+274$ \\
\hline
Mean & 81.38 & 69.93\% & $+1027$ & 62.92 & 13.24\% & $+108$ \\
SD & 1.11 & 3.33\% & 99 & 2.17 & 19.85\% & 141 \\
\hline
\end{tabular}
\end{table*}


